QMamba: Post-Training Quantization for Vision State Space Models

State Space Models (SSMs), as key components of Mamaba, have gained increasing attention for vision models recently, thanks to their efficient long sequence modeling capability. Given the computational cost of deploying SSMs on resource-limited edge devices, Post-Training Quantization (PTQ) is a technique with the potential for efficient deployment of SSMs. In this work, we propose QMamba, one of the first PTQ frameworks to our knowledge, designed for vision SSMs based on the analysis of the activation distributions in SSMs. We reveal that the distribution of discrete parameters exhibits long-tailed skewness and the distribution of the hidden state sequence exhibits highly dynamic variations. Correspondingly, we design Long-tailed Skewness Quantization (LtSQ) to quantize discrete parameters and Temporal Group Quantization (TGQ) to quantize hidden states, which reduces the quantization errors. Extensive experiments demonstrate that QMamba outperforms advanced PTQ methods on vision models across multiple model sizes and architectures. Notably, QMamba surpasses existing methods by 21.0% on ImageNet classification with 4-bit activations.

==> sec/tab_pretest.tex <==
\begin{table}[t]
  \caption{The results of quantized Vim~\cite{vim} on ImageNet classification. \emph{W32} and \emph{A32} represent full precision weights and activation, respectively. }
  % \vspace{-1.4mm}
  \tiny
  \label{tab:pretest}
  \centering
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{ccccc}
  \toprule
    \multicolumn{1}{c}{\textit{Bit}}
    &\multicolumn{1}{c}{\textit{W32A32}}
    &\multicolumn{1}{c}{\textit{W8A32}}
      &\multicolumn{1}{c}{\textit{W32A8}}
      &\multicolumn{1}{c}{\textit{W8A8}}\\ \midrule

Top-1/Top-5 (\%) &78.3/94.2 &78.1/94.1 &50.5/74.7 &49.3/73.5\\


\bottomrule
  \end{tabular}
  }
  % \vspace{-5mm}
\end{table}

==> sec/tab_vm.tex <==
% \begin{table*}[t]
%   \caption{Quantitative comparison of different PTQ method for VMamba~\cite{vmamba} on ImageNet classification. \textit{FP} means the results of the floating-point models. \textit{W8A8}, \textit{W6A6}, and \textit{W6A4} represent the bit width of weights and activations, respectively. The \textbf{best results} after PTQ are depicted in bold.}
%   % \vspace{-1.4mm}
%   \tiny
%   % \small
%   \centering
%   \label{tab:vm}
%   \resizebox{\textwidth}{!}{
%   \begin{tabular}{l|ccc|ccc|cccc}
%   \toprule
%     \multirow{3}{*}{\textit{Methods}}
%     &\multicolumn{3}{c|}{\textit{VMamba-T}}
%         &\multicolumn{3}{c|}{\textit{VMamba-S}}
%       &\multicolumn{4}{c}{\textit{VMamba-B}} \\ \cmidrule(lr){2-11}
%      &\multicolumn{1}{c}{\textit{FP}} &\multicolumn{1}{c}{\textit{W6A6}} &\multicolumn{1}{c|}{\textit{W6A4}} &\multicolumn{1}{c}{\textit{FP}} &\multicolumn{1}{c}{\textit{W6A6}} &\multicolumn{1}{c|}{\textit{W6A4}} &\multicolumn{1}{c}{\textit{FP}} &\multicolumn{1}{c}{\textit{W8A8}} &\multicolumn{1}{c}{\textit{W6A6}} &\multicolumn{1}{c}{\textit{W6A4}} \\ \midrule

% MinMax~\cite{minmax} &\multirow{7}{*}{82.6} &43.3 &5.6  &\multirow{7}{*}{83.6} &59.7 &1.2 &\multirow{7}{*}{83.9} &77.4 &52.7 &25.3 \\
% Percentile~\cite{percentile} & &63.1   &22.3 & &72.2 &29.2 & &77.0 &74.2 &46.5 \\
% OMSE~\cite{OMSE} & &65.5 &21.8  & &73.3 &10.3 & &77.3 &73.5 &46.2 \\
% AdaRound~\cite{adaround} & &71.0 &42.8  &  &77.4 &33.9 & &81.2 &79.0 &46.8 \\
% BRECQ~\cite{brecq} & &77.6 &45.6  & &80.6 &68.3 & &82.7  &81.6 &53.7 \\
% QDrop~\cite{qdrop} & &80.4 &51.9  & &82.0 &69.5  & &83.0 &82.0 &56.9 \\
% \textbf{QMamba}~(Ours) & &\textbf{80.6} &\textbf{54.9}  & &\textbf{82.3} &\textbf{71.5} & &\textbf{83.1}  &\textbf{82.1} &\textbf{60.0} \\

% \bottomrule
%   \end{tabular}
% }
% % \vspace{-4.8mm}% \vspace{-2mm}
% \end{table*}




\begin{table*}[t]
  \caption{Quantitative comparison of different PTQ method for VMamba~\cite{vmamba} on ImageNet classification. The Top-1 and Top-5 accuracy results of floating-point models are displayed below model names. \textit{W8A8}, \textit{W6A6}, and \textit{W6A4} represent the bit width of weights and activations, respectively. The \textbf{best results} after PTQ are depicted in bold.}
  % \vspace{-1.4mm}
  % \tiny
  \small
  \centering
  \label{tab:vm}
  \setlength{\tabcolsep}{1.2mm}{
  \resizebox{\textwidth}{!}{
  \begin{tabular}{c|c|ccccccc}
  \toprule
    \multirow{2}{*}{\makecell{Model \\ Top-1/Top-5 (\%)}}
    &\multirow{2}{*}{Bit}
        &\multirow{2}{*}{MinMax~\cite{minmax}}
      &\multirow{2}{*}{Percentile~\cite{percentile}} 
      &\multirow{2}{*}{OMSE~\cite{OMSE}} 
      &\multirow{2}{*}{AdaRound~\cite{adaround}}
      &\multirow{2}{*}{BRECQ~\cite{brecq}} 
      &\multirow{2}{*}{QDrop~\cite{qdrop}} 
      &\multirow{2}{*}{\textbf{QMamba}~(Ours)} 
      \\ 
      & & & & & & & & \\ \midrule

\multirow{2}{*}{\makecell{VMamba-T \\ 82.6/95.9}} 
    &W6A4 &5.6/15.7 &22.3/44.5 &21.8/43.2 &42.8/67.4 &45.6/70.6 &51.9/77.2 &\textbf{54.9/79.2}\\
    &W6A6 &43.3/67.3 &63.1/83.3 &65.5/86.1 &71.0/89.4 &77.6/93.5 &80.4/95.1 &\textbf{80.6/95.3}\\ \midrule

\multirow{2}{*}{\makecell{VMamba-S \\ 83.6/96.0}} 
    &W6A4 &1.2/3.6 &29.2/50.6 &10.3/21.1 &33.9/55.5 &68.2/87.5 &69.5/88.6 &\textbf{71.5/90.2}\\
    &W6A6 &59.7/82.6 &72.2/90.6 &73.3/90.6 &78.2/94.1 &80.6/95.3 &82.0/95.8 &\textbf{82.3/96.0}\\ \midrule

\multirow{3}{*}{\makecell{VMamba-B \\ 83.9/96.4}} 
    &W6A4 &25.3/50.1 &46.5/71.1 &46.2/71.0 &49.9/73.6 &53.7/77.3 &56.9/78.9 &\textbf{60.0/82.1}\\
    &W6A6 &52.7/75.6 &74.2/90.9 &73.5/89.4 &79.0/93.4 &81.7/95.5 &82.0/95.6 &\textbf{82.1/95.6}\\
    &W8A8 &77.4/93.5 &77.0/92.9 &77.3/92.5 &81.2/95.3 &82.7/96.2 &82.9/96.2 &\textbf{83.1/96.3}\\

\bottomrule
  \end{tabular}
}
}
% \vspace{-4.8mm}% \vspace{-2mm}
\end{table*}
